Wrench-Based Bayesian Pose Estimation via Matrix Fisher-Gaussian Inference

Estimating object position and orientation from contact forces and torques is important in robotics when vision is unavailable or unreliable. The inverse problem involves an implicit mechanical equilibrium and a nonlinear pose space. We develop a Bayesian framework for quasi-static contact measurements on ${\SO(3)}\times\mathbb{R}^3$, using a coupled Matrix Fisher--Gaussian (MFG) distribution to represent position and orientation uncertainty. The observation likelihood is generally not conjugate to this family. Implicit differentiation of the equilibrium equations yields a reduced wrench sensitivity for constructing a local quadratic model of the negative log posterior. The Coupled MFG update computes parameters of a local MFG posterior approximation in closed form by matching a conditional-mean-linearized surrogate to this model. To improve robustness to the linearization point, we introduce a residual-safeguarded refinement procedure that reuses the original prior and measurements. We establish conditional bounds on posterior approximation error and analyse the computational trade-off with particle-based inference. Numerical comparisons demonstrate computational advantages under the tested conditions. Ellipsoid and smoothed Stanford bunny simulations illustrate concentration of the fitted MFG distributions as measurements accumulate, while robotic experiments demonstrate pose estimation from contact measurements on objects with known geometry.

==> supplementary_refmap.tex <==
% Numbers and destinations from the companion document.
\makeatletter
\def\CrossDocumentSMMapVersion{20261124}
\providecommand{\SMPDFFile}{SM.pdf}
\expandafter\def\csname CrossDocumentSMnumber@alg:opt-newton\endcsname{S7.1}
\expandafter\def\csname CrossDocumentSMname@alg:opt-newton\endcsname{Algorithm}
\expandafter\def\csname CrossDocumentSManchor@alg:opt-newton\endcsname{algorithm.comparison.S7.1}
\expandafter\def\csname CrossDocumentSMnumber@app:opt-distribution-errors\endcsname{S7.4}
\expandafter\def\csname CrossDocumentSMname@app:opt-distribution-errors\endcsname{Section}
\expandafter\def\csname CrossDocumentSManchor@app:opt-distribution-errors\endcsname{subsection.7.4}
\expandafter\def\csname CrossDocumentSMnumber@app:opt-evidence\endcsname{S7}
\expandafter\def\csname CrossDocumentSMname@app:opt-evidence\endcsname{Section}
\expandafter\def\csname CrossDocumentSManchor@app:opt-evidence\endcsname{section.7}
\expandafter\def\csname CrossDocumentSMnumber@app:opt-newton\endcsname{S7.1}
\expandafter\def\csname CrossDocumentSMname@app:opt-newton\endcsname{Section}
\expandafter\def\csname CrossDocumentSManchor@app:opt-newton\endcsname{subsection.7.1}
\expandafter\def\csname CrossDocumentSMnumber@app:opt-reconstruction-cost\endcsname{S7.2}
\expandafter\def\csname CrossDocumentSMname@app:opt-reconstruction-cost\endcsname{Section}
\expandafter\def\csname CrossDocumentSManchor@app:opt-reconstruction-cost\endcsname{subsection.7.2}
\expandafter\def\csname CrossDocumentSMnumber@supp:posterior-extensions\endcsname{S6}
\expandafter\def\csname CrossDocumentSMname@supp:posterior-extensions\endcsname{Section}
\expandafter\def\csname CrossDocumentSManchor@supp:posterior-extensions\endcsname{section.6}
\expandafter\def\csname CrossDocumentSMnumber@supp:s1-geometry\endcsname{S1.1}
\expandafter\def\csname CrossDocumentSMname@supp:s1-geometry\endcsname{Section}
\expandafter\def\csname CrossDocumentSManchor@supp:s1-geometry\endcsname{subsection.1.1}
\expandafter\def\csname CrossDocumentSMnumber@supp:s1-potential\endcsname{S1.2}
\expandafter\def\csname CrossDocumentSMname@supp:s1-potential\endcsname{Section}
\expandafter\def\csname CrossDocumentSManchor@supp:s1-potential\endcsname{subsection.1.2}
\expandafter\def\csname CrossDocumentSMnumber@supp:s2-nested-results\endcsname{S2.2}
\expandafter\def\csname CrossDocumentSMname@supp:s2-nested-results\endcsname{Section}
\expandafter\def\csname CrossDocumentSManchor@supp:s2-nested-results\endcsname{subsection.2.2}
\expandafter\def\csname CrossDocumentSMnumber@supp:s2-selection\endcsname{S2.1}
\expandafter\def\csname CrossDocumentSMname@supp:s2-selection\endcsname{Section}
\expandafter\def\csname CrossDocumentSManchor@supp:s2-selection\endcsname{subsection.2.1}
\expandafter\def\csname CrossDocumentSMnumber@supp:s3-cost\endcsname{S3.1}
\expandafter\def\csname CrossDocumentSMname@supp:s3-cost\endcsname{Section}
\expandafter\def\csname CrossDocumentSManchor@supp:s3-cost\endcsname{subsection.3.1}
\expandafter\def\csname CrossDocumentSMnumber@supp:s3-probability-errors\endcsname{S3.2}
\expandafter\def\csname CrossDocumentSMname@supp:s3-probability-errors\endcsname{Section}
\expandafter\def\csname CrossDocumentSManchor@supp:s3-probability-errors\endcsname{subsection.3.2}
\expandafter\def\csname CrossDocumentSMnumber@supp:s3-reference-checks\endcsname{S3.3}
\expandafter\def\csname CrossDocumentSMname@supp:s3-reference-checks\endcsname{Section}
\expandafter\def\csname CrossDocumentSManchor@supp:s3-reference-checks\endcsname{subsection.3.3}
\expandafter\def\csname CrossDocumentSMnumber@supp:s3-sampling-diagnostics\endcsname{S3.4}
\expandafter\def\csname CrossDocumentSMname@supp:s3-sampling-diagnostics\endcsname{Section}
\expandafter\def\csname CrossDocumentSManchor@supp:s3-sampling-diagnostics\endcsname{subsection.3.4}
\expandafter\def\csname CrossDocumentSMnumber@supp:s4:apparatus\endcsname{S5.1}
\expandafter\def\csname CrossDocumentSMname@supp:s4:apparatus\endcsname{Section}
\expandafter\def\csname CrossDocumentSManchor@supp:s4:apparatus\endcsname{subsection.5.1}
\expandafter\def\csname CrossDocumentSMnumber@supp:s4:physical-validation\endcsname{S5}
\expandafter\def\csname CrossDocumentSMname@supp:s4:physical-validation\endcsname{Section}
\expandafter\def\csname CrossDocumentSManchor@supp:s4:physical-validation\endcsname{section.5}
\expandafter\def\csname CrossDocumentSMnumber@supp:s4:results\endcsname{S5.2}
\expandafter\def\csname CrossDocumentSMname@supp:s4:results\endcsname{Section}
\expandafter\def\csname CrossDocumentSManchor@supp:s4:results\endcsname{subsection.5.2}
\expandafter\def\csname CrossDocumentSMnumber@supp:sec:geometry-contact\endcsname{S1}
\expandafter\def\csname CrossDocumentSMname@supp:sec:geometry-contact\endcsname{Section}
\expandafter\def\csname CrossDocumentSManchor@supp:sec:geometry-contact\endcsname{section.1}
\expandafter\def\csname CrossDocumentSMnumber@supp:shape-clouds\endcsname{S4}
\expandafter\def\csname CrossDocumentSMname@supp:shape-clouds\endcsname{Section}
\expandafter\def\csname CrossDocumentSManchor@supp:shape-clouds\endcsname{section.4}
\expandafter\def\csname CrossDocumentSMnumber@supp:shape-geometry-controls\endcsname{S4.2}
\expandafter\def\csname CrossDocumentSMname@supp:shape-geometry-controls\endcsname{Section}
\expandafter\def\csname CrossDocumentSManchor@supp:shape-geometry-controls\endcsname{subsection.4.2}
\expandafter\def\csname CrossDocumentSMnumber@supp:tab:baseline\endcsname{S1}
\expandafter\def\csname CrossDocumentSMname@supp:tab:baseline\endcsname{Table}
\expandafter\def\csname CrossDocumentSManchor@supp:tab:baseline\endcsname{table.caption.1}
\expandafter\def\csname CrossDocumentSMnumber@supp:tab:k-rotation\endcsname{S3}
\expandafter\def\csname CrossDocumentSMname@supp:tab:k-rotation\endcsname{Table}
\expandafter\def\csname CrossDocumentSManchor@supp:tab:k-rotation\endcsname{table.caption.3}
\expandafter\def\csname CrossDocumentSMnumber@supp:tab:k-translation\endcsname{S4}
\expandafter\def\csname CrossDocumentSMname@supp:tab:k-translation\endcsname{Table}
\expandafter\def\csname CrossDocumentSManchor@supp:tab:k-translation\endcsname{table.caption.4}
\expandafter\def\csname CrossDocumentSMnumber@supp:tab:runtime-repeats\endcsname{S9}
\expandafter\def\csname CrossDocumentSMname@supp:tab:runtime-repeats\endcsname{Table}
\expandafter\def\csname CrossDocumentSManchor@supp:tab:runtime-repeats\endcsname{table.caption.12}
\newcommand{\SMNumber}[1]{%
  \ifcsname CrossDocumentSMnumber@#1\endcsname%
    \csname CrossDocumentSMnumber@#1\endcsname%
  \else%
    \PackageError{CrossDocument}{Missing SM reference: #1}{Use the paired reference map from this release.}%
    \textbf{??}%
  \fi}
% arXiv builds use versioned HTTPS links. The editable pair uses sibling PDFs.
\ifdefined\ArxivProjectDirectory\else
  \InputIfFileExists{arxiv-public-links.cfg}{}{}%
\fi
\newcommand{\CrossDocumentSMLink}[2]{%
  \ifcsname CrossDocumentSManchor@#1\endcsname%
    \ifdefined\ArxivCrossLink%
      \ArxivCrossLink{SM}{\csname CrossDocumentSManchor@#1\endcsname}{#2}%
    \else%
      \hyper@linkfile{#2}{\SMPDFFile}{\csname CrossDocumentSManchor@#1\endcsname}%
    \fi%
  \else%
    \PackageError{CrossDocument}{Missing SM PDF target: #1}{Use the paired reference map from this release.}%
  \fi}
\DeclareRobustCommand{\SMref}[1]{\CrossDocumentSMLink{#1}{\SMNumber{#1}}}
\DeclareRobustCommand{\SMeqref}[1]{\textup{\CrossDocumentSMLink{#1}{(\SMNumber{#1})}}}
\DeclareRobustCommand{\SMCref}[1]{\CrossDocumentSMLink{#1}{\csname CrossDocumentSMname@#1\endcsname~\SMNumber{#1}}}
\DeclareRobustCommand{\SMcref}[1]{\SMCref{#1}}
\makeatother

